Learning Approximately Optimal Contracts

In principal-agent models, a principal offers a contract to an agent to perform a certain task. The agent exerts a level of effort that maximizes her utility. The principal is oblivious to the agent's chosen level of effort, and conditions her wage only on possible outcomes. In this work, we consider a model in which the principal is unaware of the agent's utility and action space: she sequentially offers contracts to identical agents, and observes the resulting outcomes. We present an algorithm for learning the optimal contract under mild assumptions. We bound the number of samples needed for the principal to obtain a contract that is within $\eps$ of her optimal net profit for every $\eps>0$. Our results are robust even when considering risk-averse agents. Furthermore, we show that when there are only two possible outcomes or the agent is risk-neutral, the algorithm's outcome approximates the optimal contract described in the classical theory.

==> algorithm-backup.tex <==
\section{Main Result}
%
In this section we present our algorithm and analyze its sample complexity, but before doing so let us first define the space of contracts $W$ that we can learn. The algorithm
is presented in \cref{sec:algorithm}.
%\moran{Note that we do not present the algorithm anywhere}
%\alon{is this better?}

\subsection{Learnable Contracts}
%
Let $w_0 > 0$ be a minimum wage for any outcome.
%
\begin{definition}[$B$-bounded contract]
A contract $w$ is $B$-bounded if $w_0 \le w(i) \le B$ for every $i \in [k]$.
\end{definition}

For a bounded contract, together with the assumption that the principal's profits are bounded, ensures that the principal's expected net profit $V(w)$ can be estimated statistically. 

\begin{definition}[Monotone-smooth contract]\label{def:monotone-smooth-contract}
A contract $w$ is monotone-smooth if for every $i \in [k-1]$ it holds that $0 \le w(i+1) - w(i) \le \pi(i+1) - \pi(i)$.
\end{definition}

For a monotone-smooth contract, \cref{eq:assump} ensures that, keeping the contract fixed, 
the principal's utility cannot decrease if the agent increases her effort level. In the 
sequel, this property allows us to bound the difference in the principal's utility between 
two similar contracts.

We define $W$ as follows.
\[
W = \left\lbrace w : w~\mbox{is monotone-smooth and $H$-bounded} \right\rbrace~.
\]
%
We are aware that this set seems restrictive at first glance, yet we argue that in some important special cases, the principal's optimal net profit is achieved by a contract from this set. For example, when there are only two outcomes or the utility of the agent is linear (see \cref{sec:apps}).

\subsection{Algorithm}
\label{sec:algorithm}
%
Let $w^\star \in W$ be an optimal contract in $W$, that is $V(w^\star) \ge V(w)$ for all $w \in W$. 
The goal of our algorithm is to find an \eps-optimal contract $w$, namely a contract for which $V(w^\star) \le V(w) + \epsilon$ within a predetermined number of rounds. However, we conjecture that it cannot be done in general, and to alleviate this issue we make the following assumption.
%
\begin{assumption}[Bounded Risk-Aversion]
\label{assumption:rrn}
The agent's utility from wage $u$ is twice continuously-differentiable and satisfies $-u''(w)/u'(w) \le 1/w$ for all $w > 0$. This is equivalent to $w \mapsto w\cdot u'(w)$ being monotone-nondecreasing in $w$.
\end{assumption}
%
Intuitively, the assumption ensures that making small changes to a contract does not produce drastically different behavior by the agent. \footnote{An equivalent formulation of the assumption is that the agent's Arrow-Pratt relative risk aversion measure  is smaller than unity, i.e., $\frac{-x \cdot u''(x)}{u'(x)}<1.$  \cite{Arrow:65,Pratt1964}. When considering finite outcomes, this assumption is not very restrictive (see discussion in \cite{Arrow:65,Choi1992}).}

Our algorithm works as follows. The principal initially constructs a cover $W_\eta$ of $W$, and then run \textsc{MedianElimination} on $W_\eta$. Indeed, the main technical difficulty in this paper is in defining $W_\eta$ properly so that the following result holds.
%
\begin{theorem}
\label{thm:discretization}
Suppose that \cref{assumption:fosd,assumption:breakties,assumption:rrn} hold. Let $\eta < 1/4k$. There exists a contract space $W_\eta$ such that for every contract $w \in W$, there is a contract $w' \in W_{\eta}$ for which $V(w) \le V(w') + 2 k H \eta$. Moreover, the size of $W_{\eta}$ is at most $M = (\log(2H/w_0) / \eta)^k$, and $W_\eta$ can be constructed in time $O(k M)$.
\end{theorem}

The proof of the theorem is found in \cref{sec:discproof}. Finally, we have our main result.
%
\begin{theorem}
\label{thm:main}
Suppose that \cref{assumption:fosd,assumption:breakties,assumption:rrn} hold. 
%
Let $\eta = \eps/4kH$.
Executing \textsc{MedianElimination}$(\epsilon/2,\delta)$ on the set $W_{\eta}$ produces the following guarantee. With probability at least $1-\delta$, the algorithm outputs an $\eps$-optimal contract after 
\[
O \left( \left(\frac{4kH \log (H/w_0)}{\eps} \right)^{k+2} \log(1/\delta) \right)
\]
rounds.
\end{theorem}

\begin{proof}
By \cref{thm:discretization} and by the choice of $\eta$, there is a $w' \in W_{\eta}$ for which $V(w') \le V(w^\star) + \eps/2$.
By \cref{thm:me}, with probability $1-\delta$, \textsc{MedianElimination} returns a contract $\hat w \in W_{\eta}$ such that $V(\hat w) \le V(w') + \eps/2$. Combining both results we get
\[
V(\hat w) \le V(w')+\eps/2 \le V(w^\star) + \eps/2 + \eps/2 = V(w^\star) + \eps~,
\]
as required. Moreover, \textsc{MedianElimination} is done in the following number of rounds:
\[
O \left( \frac{|W_{\eta}| H^2}{(\eps/2)^2} \log(1/\delta) \right) = O \left( \left(\frac{4kH \log (H/w_0)}{\eps} \right)^{k+2} \log(1/\delta) \right)~.\qedhere
\]
\end{proof}

\subsection{Discretization of the Contract Space}
\label{sec:discproof}
In this section we prove \cref{thm:discretization}. We start by defining the notion of a coarse contract.

\begin{definition}[$\eta$-coarse contract]
A contract $W$ is $\eta$-coarse if there exists natural numbers $l_0,l_1,\ldots,l_{k-1}$ such that $w(1) = w_0 \exp(\eta \cdot l_0)$, and for $i \in [k-1]$, $w(i+1) = w(i) \exp(\eta \cdot l_i)$.
\end{definition}
%
That is, a coarse is a contract in which the ratios between wages of consecutive outcomes come from a discrete set of options. We define:
\[
W_\eta = \left\lbrace w : w~\mbox{is $\eta$-coarse and $2H$-bounded} \right\rbrace~.
\]
%
We prove the following.
\begin{lemma}
The size of $W_\eta$ is at most $M = (\log(2H/w_0)/\eta)^k$. Moreover, $W_\eta$ can be constructed in time $O(k M)$.
\end{lemma}

\begin{proof}
The wage of outcome $i$ has the form $w_0 \exp(\eta \cdot l)$ for a natural number $l$, and satisfies $w(i) \le 2H$. Therefore, the number of choices for $w(i)$ is at most $\log(2H/w_0)/\eta$. Since there are $k$ outcomes, there must be at most $M$ such contracts.
%
To construct $W_\eta$ we can go over all of its elements one-by-one, which takes $O(M)$ time.
\end{proof}

Finally let $w \in W$, we need to show that there is $w' \in W_\eta$ such that $V(w) \le V(w') + 2kH\eta$. We construct $w' \in W_\eta$ as follows.
We let $l_0 = \lceil \log(w(1)/w_0)/\eta \rceil$, and for $i \in [k-1]$, $l_i = \lceil \log(w(i+1)/w(i))/\eta \rceil$. We can immediately observe that, by construction, $w'(1) \ge w(1)$ and for $i \in [k-1]$, we have $w'(i+1)/w'(i) \ge w(i+1)/w(i)$. Moreover, it is clear that $w'$ is $\eta$-coarse and that $w'(i) \ge w_0$, yet it remains to show that $w'(i) \le 2H$. For that, we have the following lemma.
%
\begin{lemma}
\label{lemma:discwageub}
We have for all $i \in [k-1]$, $w'(i) \le e^{\eta i} w(i)$.
\end{lemma}
%
\begin{proof}
By construction, for each $i \in [k-1]$ we have $w'(i+1)/w'(i) \le e^\eta \cdot w(i+1) / w(i)$. From this we entail that $w'(i)/w'(1) \le \exp((i-1) \cdot \eta) \cdot w(i) / w(1)$. Since also by construction $w'(1) \le \exp(\eta) \cdot w(1)$, we get that $w'(i) \le \exp(i \cdot \eta) \cdot  w(i)$ as required.
\end{proof}
%
With the lemma at hand, and by assumption that $\eta < 1/2k$ we obtain
\[
w'(k) \le \exp(\eta \cdot k) \cdot w(k) \le e^{1/2} H \le 2H~.
\]
Therefore we have $w' \in W_\eta$.

We now show that, compared to $w$, under $w'$ the agent's effort 
cannot decrease. Then, we use this fact to bound the difference in the principal's utility between $w$ and $w'$.

In order to prove our first claim, we will make use of the following lemma.
%
\begin{lemma}[\cite{Grossman1983}]
\label{lem:G83}
Let $w^1$ and $w^2$ be contracts. Then,
\begin{align*}
\sum_{i=1}^k \left(f_{\hat e(w^1)}(i) - f_{\hat e(w^2)}(i)\right) \cdot \big(u(w^1(i)) - u(w^2(i)) \big) \ge 0.
\end{align*}
\end{lemma}

\begin{lemma}
\label{lem:lplus}
The effort level the agent chooses can only increase from $w$ to $w'$.
\end{lemma}
%
\begin{proof}
First, notice that since the wages only increase, had the agent accepted the contract $w$, 
i.e., chose an effort level different than 0, she would also accept contract $w'$. So, let 
$e' = \hat e(w')$ and $e = \hat e(w)$ be the effort levels the agent chooses under contracts $w'$ and $w$ respectively.

If we apply Lemma~\ref{lem:G83} with $w$ and $w'$, we obtain
\begin{align*}
\sum_{i=1}^k \big(f_{e'}(i) - f_{e}(i)\big)\cdot \left(u(w'(i)) - u(w(i)) \right) \ge 0~.
\end{align*}
Assume for now that $u(w'(i)) - u(w(i))$ is monotone nondecreasing in $i$. Given this, we will show by contradiction that $e' \succ e$. So, for the sake of contradiction assume that
$e' \prec e$. From the fact that $f_{e}$ dominates $f_{e'}$, \cref{eq:assump} implies that
\begin{align*}
\sum_{i=1}^k \big(f_{e'}(i) - f_{e}(i)\big) \cdot \big(u(w'(i)) - u(w(i)) \big) \le 0~.
\end{align*}
Thus,
\begin{align}
\label{eq:help}
\sum_{i=1}^k \left(f_{e'}(i) - f_{e}(i)\right) \cdot u(w(i)) = \sum_{i=1}^k \left(f_{e'}(i) - f_{e}(i)\right) \cdot u(w'(i)).
\end{align}
Therefore, by optimality of $e$ and $e'$ under contracts $w$ and $w'$ respectively, 
we obtain
\begin{align*}
%\label{eq:help2}
\sum_{i=1}^k \big(f_{e'}(i) - f_{e}(i)\big) \cdot u(w(i)) \le c(e') - c(e),~\text{and}~
\sum_{i=1}^k \big(f_{e'}(i) - f_{e}(i)\big)\cdot u(w'(i)) \ge c(e') - c(e).
\end{align*}
Combining \cref{eq:help} with the two inequalities above, we obtain that 
\[
U(w',e') = \sum_{i=1}^k f_{e'}(i) \cdot u(w'(i)) - c(e') = \sum_{i=1}^k f_{e}(i) \cdot u(w'(i)) - c(e) = U(w',e)~.
\]
This means that the agent is indifferent between effort levels $e$ and $e'$ under contract 
$w'$. Since, by \cref{assumption:breakties}, the agent chooses the highest effort in this case, we must have 
$e \prec e'$ --- a contradiction.

Hence, in order to prove the lemma it suffices to prove that $u(w'(i)) - u(w(i))$ is monotone nondecreasing in $i$. 
This is equivalent to showing that $u(w'(i+1))-u(w'(i)) \ge u(w(i+1)) - u(w(i))$. 
Denote $c = w'(i)/w(i)$, for $c \ge 1$. By construction, $w'(i+1) / w(i+1) \ge c$. 
Consequently, since $u$ is monotone nondecreasing, it suffices to show $u(c \cdot w(i+1)) - u(c \cdot w(i)) \ge u(w(i+1)) - u(w(i))$.

Thus, the proof boils down to showing $c \mapsto u(c \cdot w(i+1)) - u(c \cdot w(i))$ is monotone nondecreasing in $c$. Taking the derivative with respect to $c$, we need to show
\[
u'\big(c \cdot w(i+1)\big) \cdot w(i+1) - u'\big(c \cdot w(i)\big) \cdot w(i) \ge 0.
\]
However, since the agent is BRA (\cref{assumption:rrn}), we have 
$u'\big(c \cdot w(i+1)\big)\cdot c \cdot w(i+1) \ge u'\big(c \cdot w(i)\big) \cdot c \cdot w(i)$. The proof is complete by recalling that $c \ge 1$.
\end{proof}

We can now bound the loss the principal suffers when she offers $w'$ instead of $w$.

\begin{lemma}
\label{lem:regret-bound}
It holds that $V(w) \leq V(w') + 2kH\eta$.
\end{lemma}
%
\begin{proof}
Since we focus on scenarios where the optimal contract is monotone-smooth, we get that the net profit of the principal at the optimal contract, $\pi(i) - w(i)$, is nondecreasing in $i$.
Furthermore, from \cref{eq:assump}, keeping $w$ fixed, the principal only benefits from an increase of the agent's effort level. Denote $e = \hat e(w)$ and $e' = \hat e(w')$. From \cref{lem:lplus} we know that  $e' \succ e$. We have,
\begin{align}
V(w) &= \sum_{i=1}^k f_{e}(i) \cdot \big(\pi(i) - w(i) \big) \nonumber \\
&\le \sum_{i=1}^k f_{e'}(i) \cdot \big( \pi(i) - w(i) \big) \nonumber \\
&= V(w') + \sum_{i=1}^k f_{e'}(i) \cdot  \big(w'(i) - w(i) \big).
\label{eq:principalutilitybound}
\end{align}
%
Now by \cref{lemma:discwageub}, $w'(i) \le e^{i \cdot \eta} \cdot w(i)$ for all $i \in [k]$. Since $e^x -1 \le 2x$ for all $x \in [0,1]$ and since $\eta < 1/k$, we obtain 
\[
w'(i) - w(i) \le (e^{i\cdot \eta} - 1) \cdot w(i) \le 2 \cdot \eta \cdot i \cdot w(i) \le 2 \cdot \eta \cdot k \cdot H~.
\]
Combining the latter with \cref{eq:principalutilitybound}, we get 
$V(w) \le V(w') + 2 \cdot \eta \cdot k \cdot H$.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> intro.tex <==
\section{Introduction}




Recent technological advances have had a profound impact over the relationship between firms and employees. The rapid change in employees' required skill set combined with the availability of off-shore, qualified, cheaper hiring alternatives drove employers to adopt employees on a short-term, task specific bases. This hiring model, dubbed \textit{dynamic workforce} or \textit{gig-economy} has been growing exponentially over the past couple of years and \cite{Bughin2016} found that 20-30\% of US workers are employed independently, at least partly, and predicts this trend will continue with popularity of the ``Lean Startup'' business model, and the appearance of platforms such as ``Amazon Mechanical Turk''.

The aforementioned changes in the labor market have a profound effect on the information  available to firms when it makes a hiring decision.
%relationship between managers and workers.\alon{repeated from last paragraph}
In the traditional workspace, hiring is often a long-term, expensive procedure. Nowadays hiring is cheap and short-termed. As a result, a manager has less information on the character and quality of her employees, thus lacking the knowledge on how to best align their incentives with those of the firm.  
Unfortunately, the vast majority of economic literature on such scenarios, dubbed the \textit{agency problem}, assumes that the manager (a.k.a the principal) has profound knowledge over his workers' (a.k.a the agents) incentive structure. %\argy{Do we want this here?}\moran{I think we need to say something about why this model is relevant now...so I vote yes - Alon?} 
\alon{changed my mind, we should remove this line as it is repeated in the next paragraph. }\moran{I disagree - it is the best place to state our theoretical claim, even if it is repetitive, we need to say this right here. Next paragraph we elaborate on it.}\alon{Argy, a penny for your thoughts}
In this work we attempt to construct a model more suitable to the new ``dynamic workforce''. We propose a set of contracts that the manager can learn without assuming any specific agent utility function and present cases in which the net profit under a learned contract approximates the net profit under the theoretically optimal contract. \alon{we use manager instead of principal sometimes. We should be consistent.}\moran{Is it better now?}\alon{We use principal everywhere else. I think we should stick with principal.}

%In the Economics literature, agency problems describe situations in which one party, \alon{once again repetition from the last paragraph.}
%the {\em principal}, offers a {\em contract} to another party, the {\em agent}, to 
%perform a task~\citep{laffont2009}.  % with a stochastic outcome.  
The study of agency problems emerged as one of the pillars of information economics.  
In his seminal paper, \cite{Ross1973} introduced the term {\em principal--agent}, 
to  capture the aforementioned model. In the basic model, the outcome of the task is chosen randomly from a distribution determined by the {\em level of effort} invested by the agent. A higher effort level induces a distribution in which the probability of a better outcome is higher than in lower effort levels. On the other hand, a higher level causes the agent greater disutility.    
\cite{Ross1973} assume that the principal is {\em risk-neutral} while the agent is {\em risk-averse}, therefore the incentives of both parties are {\em not} fully aligned.\footnote{When given the choice between participating in some lottery $X$ or receiving $E(X)$ with probability one, a risk-averse agent will strictly prefer the latter while a risk-neutral agent is indifferent. In the Von Neumann Morgenstern utility theory, if an agent is risk-averse, then she has a concave utility function; if she is risk-neutral, then her utility is linear.} Hence, the effort level that is optimal from the perspective of the principal, is not necessarily the optimal one for the agent. To bridge this gap, the principal offers the agent a contract in which the agent is rewarded for any additional effort. %\cite{Ross1973} proved that cases in which  compares two scenarios: 
%(1) The principal observes the effort level chosen by the agent; \alon{Is this relevant? should we even mention this?}
%(2) The principal observes only the realized outcome. 
%In the first case, the principal can condition the payment on the effort level the agent chooses (perfect monitoring), while in the other one, she can condition the payment \emph{only} on the realized outcome. In both cases, there exists an \emph{optimal} contract for the principal; a contract that maximizes her net profit. However, the net profit under the optimal contract for the first scenario is always higher than the one for the second scenario.
The lion's share of previous work assumed that the principal, while oblivious to the agent's choice, has full information about the agent's utility structure {\em and} the set of levels of effort she can choose from {\em and} the probability distribution associated with every level of effort \citep{Ross1973,Grossman1983,Holmstrom1979,Gershkov2012,Holmstrom2017} \alon{repetition from some paragraphs ago}\moran{for emphasis - I removed one place in which they repeated...}. These assumptions seem confining, especially when considering the scenario of a dynamic workplace mentioned above.% where agents are hired for an extremely short period of time, often from a long distance.  In this setting, the principal has limited familiarity with the agents' character and abilities.  \alon{repetition}
%These scenarios are gaining traction with the increase 

\cite{Holmstrom2017} identified this gap in theory as one of the main challenges in current research. \cite{Ho2016} were among the first who tried to bridge this gap. 
They considered a setting where there are several types of agents, each one with her own utility function, set of effort levels and effort costs, and probability distributions over the outcomes; all of which unknown to the principal. They considered a repeated setting with $T$ periods, where in every period the type of the agent was chosen i.i.d. from an unknown probability distribution. 
Their goal was to find, before period $T$, the optimal contract in a finite set $S$ of predefined contracts. 
%They assumed that the {\em actual} optimal contract is {\em monotone}, i.e, the payment to the agent for a better outcome is higherthan the payment for a lower outcome, and $S$ contained the se  
They followed a multi-armed bandit \citep{robbins1985some} approach and derived an algorithm that finds an approximately optimal contract. However, the contract they find is approximately optimal {\em only} with respect to the optimal contract from $S$. They provide no theoretical guarantees on approximating the optimal contract overall. In addtion, their  theoretical bound is studied only for the case of one effort level for the agent, i.e. reject the contract or accept it, known as {\em dynamic pricing}.\footnote{ As they highlight, it is not generally unclear whether the best contract from $S$ can provide a good theoretical guarantees for the general problem of dynamic contract design.} 

%A first attempt to bridge this gap was \cite{Carroll2015}, who present a model where the principal has only partial knowledge of the agent's action space. He assumes the agent is risk neutral and thus, if the principal have known the Agent's complete action space, the optimal contract would have been linear. 
%In this setting, the principal can derive the optimal linear contract only with respects to the subset of the agent's actions she knows. \cite{Carroll2015} shows that her profit from the actual action taken by the agent (which can be an action in the subset the principal is unaware of)  can only be higher than the principal's expectations. 

In this paper we follow a similar route to~\cite{Ho2016}. We assume the principal has {\em zero} information about the agent; we assume unknown utility for the agent, unknown set of effort levels and their associated costs, and unknown probability distribution for any effort level. 
The only knowledge the principal has is the set of outcomes and their corresponding profits. Our goal is to learn an {\em approximately}-optimal contract for the principal when she faces a stream of different, but identical (in terms of utility, effort levels, effort costs, and probability distributions), agents. \alon{repetition again, and we are about to say the same in the contributions part.}

\paragraph{\bf Our contribution.}
We show how to learn an \eps-optimal contract, for 
any $\eps>0$, under some assumptions about the optimal contract and the  utility function of the agent; a contract is \eps-optimal if there is no other contract such that the net profit of the principle can increase more than \eps \alon{Probably skip the formal definition of \eps-optimality to the prelims...}. To achieve this, we firstly introduce {\em monotone-smooth} contracts.
A contract is monotone if the payment to the agent for a better outcome is higher than the payment for a lower outcome--~\cite{Ho2016} assume that the optimal contract is monotone. Furthermore, their finite set of contracts contained only monotone contracts. A monotone-smooth contract is a monotone contract, where the difference between the payments for two outcomes is bounded by the difference of the value of the principal for these outcomes.\alon{we should probably skip the formal definitino of monotone-smoothness and just say its a large subset of monotone contracts ho et al. considers.} When there are only two outcomes, \cite{Grossman1983} showed that the optimal contract is monotone-smooth.
We complement this definition of a careful discretization of the contract space.
%
We show that for any monotone-smooth contract, if the utility 
function of the agent is {\em bounded 
risk-averse}, there exists a contract on the discretized space for which the principal's expected net profit is 
$\eps$-approximated. This allows to apply machineries from multi-armed bandit theory and find an $\eps$-optimal contract. Recall, in the setting we focus our approach guarantees to find a contract with approximately optimal net profit for the principal against 
{\em any} contract the principal can offer.\alon{I say remove this sentence..} To the best of our knowledge, this is the 
first work that can offer such a theoretical guarantee. 

% We limit the set of contract to ``affine contract", that is contracts in which the agent receives a base pay, plus an additional share of the income for high rewards.   Our theoretical findings prove that an approximate optimal can be learned when \moran{in polynomial time?} when  there are two possible outcomes \moran{Do we need the assumption of $R<1$ for the two outcome case?} , or  when the agent is risk neutral (as in \cite{Carroll2015}). 

\paragraph{\bf Further related work.} 
Our work lies in the intersection of principal-agent models %
%where the principal has limited, or zero, information about the agent 
and multi-armed bandit theory; 
\cite{Ho2016} provide an excellent overview of literature in the field.
\cite{Sannikov08,Sannikov11,williams2004} study a repeated setting where the principal interacts with the agent for multiple periods.
\cite{Conitzer2006} empirically compare several learning algorithms in a setting similar to~\citep{Ho2016}. 

The Lipschitz Bandit problem \citep{agrawal1995continuum} is a generalization of the multi-armed bandit problem in which the set of arms comes from some compact space, and the expected reward of each arm is a Lipschitz function of the arm. It has received much attention from the bandit theory community over the years \citep{kleinberg2005nearly,auer2007improved,bubeck2011lipschitz,kleinberg2013bandits,magureanu2014lipschitz}. 

The technique was used in the seminal paper of \cite{kleinberg2003value} for learning posted-price auctions, which can be seen as a principal-agent problem with only one outcome. There is a flourish of studies on learning auctions~\citep{BDH+17,Blum2004,BSV16,Cole2014,E07,Gonczarowski2016,MT16,RS16,S17}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
